Development of Cognitive Intelligence in Pre-trained Language Models

Recent studies show evidence for emergent cognitive abilities in Large Pre-trained Language Models (PLMs). The increasing cognitive alignment of these models has made them candidates for cognitive science theories. Prior research into the emergent cognitive abilities of PLMs has largely been path-independent to model training, i.e., has focused on the final model weights and not the intermediate steps. However, building plausible models of human cognition using PLMs would benefit from considering the developmental alignment of their performance during training to the trajectories of children's thinking. Guided by psychometric tests of human intelligence, we choose four sets of tasks to investigate the alignment of ten popular families of PLMs and evaluate their available intermediate and final training steps. These tasks are Numerical ability, Linguistic abilities, Conceptual understanding, and Fluid reasoning. We find a striking regularity: regardless of model size, the developmental trajectories of PLMs consistently exhibit a window of maximal alignment to human cognitive development. Before that window, training appears to endow "blank slate" models with the requisite structure to be poised to rapidly learn from experience. After that window, training appears to serve the engineering goal of reducing loss but not the scientific goal of increasing alignment with human cognition.

==> tex/SAT_ques.tex <==
\begin{table*}[!ht]
    \centering
    \caption{Accuracy of the PLMs Scholastic assessments tests (SAT) analogy questions. Each question has five options so the random chance }
    \label{tab:sat}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lccc:cccc:c}
    \hline
     Model &\multicolumn{3}{c:}{\begin{tabular}[c]{@{}c@{}}  Latent Representations  \end{tabular}}    & \multicolumn{4}{c:}{\begin{tabular}[c]{@{}c@{}}  Surprisal Values  \end{tabular}}  & Prompting \\ 
       
       & 3-cos-add & 3-cos-mul & Concat cos & Zero-shot & One-shot& Two-shot & Three-shot & \\ \hline
        Amber-7B & 0.217 & 0.209 & 0.283 & 0.126 & 0.139 & 0.128 & 0.131  & NA\\ \hdashline
        Falcon-7B & 0.289 & 0.267 & 0.294 & 0.142 & 0.131 & 0.118 & 0.107 & NA\\ \hdashline
        Starling-LM-7B-alpha & 0.238 & 0.235 & 0.313 & 0.142 & 0.126 & 0.115 & 0.126 & NA \\ \hdashline
        Llama-2-7B & 0.238 & 0.209 & 0.302 & 0.099 & 0.131 & 0.110 & 0.102 & NA\\ 
        Llama-2-13B & 0.203 & 0.193 & 0.302 & 0.115 & 0.112 & 0.099 & 0.102 & NA\\ \hdashline
        Mistral-7B & 0.246 & 0.222 & 0.302 & 0.139 & 0.120 & 0.118 & 0.107 & NA \\ 
        Mistral-7B-Instruct & 0.222 & 0.217 & 0.278 & 0.136 & 0.123 & 0.120 & 0.102 & NA \\ \hdashline
        Qwen-0.5B & 0.278 & 0.238 & 0.283 & 0.136 & 0.134 & 0.150 & 0.147 & NA \\ 
        Qwen-1.8B & 0.230 & 0.209 & 0.259 & 0.139 & 0.152 & 0.150 & 0.139 & NA\\ 
        Qwen-4B & 0.238 & 0.225 & 0.332 & 0.107 & 0.155 & 0.115 & 0.118 & NA\\ 
        Qwen-7B & 0.267 & 0.238 & 0.307 & 0.142 & 0.155 & 0.136 & 0.128 & NA\\ 
        Qwen-14B & 0.211 & 0.225 & 0.273 & 0.158 & 0.126 & 0.104 & 0.086 & NA\\ \hdashline
        Pythia-70M & 0.209 & 0.184 & 0.217 & 0.171 & 0.152 & 0.168 & 0.150 & NA \\ 
        Pythia-160M & 0.203 & 0.198 & 0.246 & 0.158 & 0.155 & 0.134 & 0.139 & NA\\ 
        Pythia-410M & 0.230 & 0.238 & 0.259 & 0.171 & 0.128 & 0.139 & 0.144 & NA\\ 
        Pythia-1B & 0.257 & 0.238 & 0.278 & 0.160 & 0.144 & 0.160 & 0.142 & NA\\ 
        Pythia-1.4B & 0.214 & 0.246 & 0.246 & 0.144 & 0.139 & 0.144 & 0.139 & NA\\ 
        Pythia-2.8B & 0.241 & 0.251 & 0.267 & 0.150 & 0.147 & 0.134 & 0.136 & NA\\ 
        Pythia-6.9B & 0.235 & 0.233 & 0.262 & 0.118 & 0.179 & 0.171 & 0.139 & NA\\ 
        Pythia-12B & 0.233 & 0.227 & 0.241 & 0.126 & 0.160 & 0.147 & 0.131 & NA \\ \hdashline
        Gemini & NA & NA & NA & NA & NA & NA & NA & 0.781 \\ \hdashline
        GPT-3.5-Turbo & NA & NA & NA & NA & NA & NA & NA & 0.799 \\
        GPT-4 & NA & NA & NA & NA & NA & NA & NA & 0.804 \\ \hline
    \end{tabular}
    }
\end{table*}
